ENTRUST: Argument Reframing with Language Models and Entailment

Framing involves the positive or negative presentation of an argument or issue depending on the audience and goal of the speaker (Entman 1983). Differences in lexical framing, the focus of our work, can have large effects on peoples' opinions and beliefs. To make progress towards reframing arguments for positive effects, we create a dataset and method for this task. We use a lexical resource for "connotations" to create a parallel corpus and propose a method for argument reframing that combines controllable text generation (positive connotation) with a post-decoding entailment component (same denotation). Our results show that our method is effective compared to strong baselines along the dimensions of fluency, meaning, and trustworthiness/reduction of fear.

==> comments.tex <==
Line 166
%TC TODO : Motivate why retrieval wont work better maybe idk
%CH - we could say the retrieve and replace methods make it difficult to get both syntax/fluency and semantics correct
%CH - took a stab at editing the commented part, feel free to change back
%Retaining the semantics and enforcing a strict control for our generative models is extremely necessary for this task. Our experiments in Section \ref{section:exp} later show how retrieval based approaches are not suitable for this task as the attributes even though localized to a small fraction of the words is very much dependent on broader context of sentences and differ significantly from other attribute transfer tasks such as sentiment \cite{li2018delete,sudhakar2019transforming}. This makes style transfer with supervision necessary.


% \begin{table}[]
% \small
% \centering
% \begin{tabular}{|l|l|}
% \hline
% Source & \begin{tabular}[c]{@{}l@{}} \textbf{\color{blue}joy:trust} {[}DELIM{]} Nation states have\\ incredible {[}SEP{]} tools {[}SEP{]} available for\\ espionage\end{tabular} \\ \hline
% Target & \begin{tabular}[c]{@{}l@{}}Nation states have incredible resources\\ available  for espionage\end{tabular}                                      \\ \hline
% \end{tabular}
% \caption{A sample pair from our parallel data for rewriting arguments. ``Source'' is the premise edited by an MLM while ``Target'' is the original premise}
% \label{table:source-target}
% \end{table}


%CH - tried to make some edits here, original commented
%To re-write arguments then we take the premise with replacements from MLM as the source side of the parallel data while the original premises are treated as target as shown in Table \ref{table:source-target}. Recent work has used Aspect as a control code \cite{keskar2019ctrl} for Argument Generation \cite{schiller2020aspect}. Motivated by this we also concatenate the emotional associations of the words from the connotation dictionary and add as control code \cite{keskar2019ctrl} at the beginning of our source. This helps us tune the emotion of the rewritten argument at inference time or decoding. In order to ensure better controllability we also add [SEP] tokens at the boundary of the words we aim to replace to provide our generative model with a better signal on what to replace or rewrite. 


%CH - maybe we should say something here about how this has the potential downside of needing to identify spans for replacement, but our approach (using collocations or fear words) makes it unneccessary 


%  \footnote{\url{https://www.reddit.com/r/changemyview/}}
% \footnote{\url{https://www.reddit.com/r/politics/}}


%CH - did we use the AMPERSAND model for classification?
%TC yes

%CH - maybe can add ``


\begin{comment}
\begin{table*}[]
\centering
\small
\begin{tabular}{|l|l|l|l|l|}
\hline
System  & Text                                                                                                                                                                                    & F & M & PF \\ \hline
INPUT   & A campaign of \text{\color{red} hate} laced with \text{\color{red} blatant} anti-semitic overtones                                                                                                                                & -  & - & 2.7   \\ \hline
BART$^{w/o}_{D+EN}$   & A campaign of \text{\color{red} hate} laced with \text{\color{blue} genuine} anti-semitic overtones                                                                                                                           & \textbf{4.3}  &  \textbf{4.7}  & 2.3   \\ \hline
BART$^{w/o}_{EN}$   & A campaign of \text{\color{blue} trust} laced with \text{\color{blue} obvious} anti - semitic overtones                                                                                                                                   & 2.0  & 1.7  &  \textbf{2.0}   \\ \hline
LEXREP  & A campaign of \text{\color{blue}intimidation} laced with \text{\color{blue}strong} anti-semitic overtones                                                                                                                                & 3.3  &  3.0  &  \textbf{2.0}  \\ \hline
GST     & \begin{tabular}[c]{@{}l@{}}A campaign of \textit{\color{blue}injuring rollercoaster} laced with anti - semitic overtones\end{tabular}                                               & 2.3  & 1.0  &  \textbf{2.0}   \\ \hline
ENTRUST & A campaign of \text{\color{blue} prejudice} laced with \text{\color{blue} genuine} anti-semitic overtones                                                                                                                      & 3.7  & 4.0  & \textbf{2.0}   \\ \hline
HUMAN   & \begin{tabular}[c]{@{}l@{}}A campaign with \textit{\color{blue}clear} anti-semitic overtones which \textit{\color{blue}does not promote peace}\end{tabular}                                                                                                                   & 2.7  & 2.7  &  3.7  \\ \hline\hline
INPUT   & \begin{tabular}[c]{@{}l@{}}Or he can \textit{\color{red}seize} this opportunity and use his \textit{\color{red}government's} diplomatic \textit{\color{red}influence} to\\ \textit{\color{red}defend} the life of an australian citizen , whose \textit{\color{red}courageous} public service is \\recognised by countless people across the world\end{tabular}              &   -&  - &  \textit{2.3}  \\ \hline
BART$^{w/o}_{D+EN}$   & \begin{tabular}[c]{@{}l@{}}Or he can \textit{\color{red}seize} this opportunity and use his \textit{\color{red}governments's} diplomatic \textit{\color{red}influence} to\\ \textit{\color{red}defend} the life of an australian citizen , whose courageous \textit{\color{blue} military} service is \\recognised by countless people across the world\end{tabular}                &  2.7 & 3.0  &  3.0  \\ \hline
BART$^{w/o}_{EN}$   & \begin{tabular}[c]{@{}l@{}}Or he can \textit{\color{blue}honor} this opportunity and use his \textit{\color{blue}nations's} diplomatic \textit{\color{blue}resources} to\\ \textit{\color{red}defend} the life of an australian citizen , whose courageous \textit{\color{blue} military} service is \\recognised by countless people across the world\end{tabular}         & 4.0  &  4.7 &  \textbf{2.3}  \\ \hline
LEXREP  & \begin{tabular}[c]{@{}l@{}}Or he can \textit{\color{blue}take} this opportunity and use his \textit{\color{blue}considerable} diplomatic \textit{\color{blue}clout} to\\ \textit{\color{blue}save} the life of an australian citizen , whose \textit{\color{blue}heroic} public service is \\recognised by countless people across the world\end{tabular}            & \textbf{4.7}  & 4.0  &    \\ \hline
GST     & \begin{tabular}[c]{@{}l@{}}Or he can \textit{\color{blue}do} this opportunity and use his diplomatic \textit{\color{blue}expertise} to \textit{\color{blue}change} the life of an\\ australian citizen , whose public service is recognised by countless\\ white people across the world.\end{tabular}          &  1.7 & 2.0  &    \\ \hline
ENTRUST & \begin{tabular}[c]{@{}l@{}}Or he can \textit{\color{blue}honor} this opportunity and use his \textit{\color{blue}nation's} diplomatic \textit{\color{blue}resources} to\\ \textit{\color{blue}vindicate} the life of an australian citizen , whose \textit{\color{blue}unwavering} public service is \\recognised by countless people across the world\end{tabular}           & \textbf{4.7}  & \textbf{4.7}  &    \\ \hline
HUMAN   & \begin{tabular}[c]{@{}l@{}}Or he can \textit{\color{blue}pick up} this opportunity and use his government ’s diplomatic influence to\\ defend the life of an australian citizen , whose \textit{\color{blue}actions have been publicly recognized as} \\\textit{\color{blue}highly relevant at an international level}. 
\end{tabular} & 3.7  & 4.0  &    \\ \hline
\end{tabular}
\caption{Examples of generated outputs from different systems (with human re-framed argument as references) for arguments containing appeal to Fear or Prejudice. We show average scores (over three annotators) on a 1-5 scale with 1 denotes the worst and 5 be the best.}
\label{table:fear}
\end{table*}
\end{comment}

==> related_work.tex <==
%TODO argumentation and propaganda

The effects of lexical framing have been studied for social and political issues, although our work is the first to use lexical framing in generation for positive framing effects. \citet{demszky2019analyzing} and \citet{tyagi2020computational} study political polarization and how this manifests in differences in word choice among different groups; \citet{khudabukhsh2020we} provide an interpretable framework using machine translation between groups to generate differences.
While these works encourage computational approaches  to reframe arguments for better lexical choice, these approaches do not control for denotation or connotation and thus may cause differences in word choice to result in a change in meaning.
The most similar work to ours is that of \citet{pryzant2020automatically}, who use a corpus of Wikipedia edits to train a model for debiasing, which includes framing.
However, in their work communicative intent is left implicit; the corpus is only labeled for types of debiasing, which includes framing at a high level and not the connotations involved. Thus, their model only learns lexical differences whereas our model is controllable.  

While our focus is on lexical framing, other work has investigated the identification of other types of frames and their effects. \newcite{greene-resnik-2009-words} studied \textit{syntactic} framing, finding a link between implicit sentiment and syntactic packaging (e.g. the difference between active and passive voice). Previous studies have also involved \textit{emphasis} framing -- \newcite{ding-pan-2016-personalized} find that emphasizing aspects of products given personal information is more effective for content selection in advertisements. Other research has involved \textit{issue} framing -- \newcite{ajjour-etal-2019-modeling} and \newcite{hartmann-etal-2019-issue} study how arguments are framed in debates (e.g. in terms of economics, feasibility, and safety). \citet{Nguyen2013LexicalAH} and \citet{field2018framing} study ``agenda-setting'' for news and congressional debates and \newcite{DBLP:journals/pacmhci/AugustOTSR18} for study recruitment. \newcite{cano-basave-he-2016-study} and \newcite{Musi2019FramingFS} leverage \textit{semantic} frames for distant labeling and analysis of arguments in political debates, respectively, and find, for example, that evidence and reasoning are among the most common. 

Finally, our work is also related to style transfer and controllable generation. Much of the work in ``style transfer'' has referred to changing the sentiment of a statement, which changes the truth condition and thus the denotative meaning. Sentiment is often explicitly marked and thus approaches such as deleting and replacing lexical markers are effective \cite{li-etal-2018-delete, sudhakar-etal-2019-transforming}, although our experiments showed the difficulty of applying these techniques to our task.
To control text generation by limiting contradictions, \citet{pasunuru2017reinforced} use an entailment score as a reward in Reinforcement Learning, ensuring that a generated text is logically implied (i.e., is a paraphrase or directed partial match with) by the ground-truth text. \citet{holtzman2018learning} utilize a discriminative model trained on SNLI \cite{bowman2015large} to complement an RNN generator and guide the decoding process to improve contradictions in generation. Although we experimented with both these approaches, including the approach of \citet{holtzman2018learning}  with MNLI to account for entailment in text generation, none of them yielded better results than our method. Other approaches have explored ``vocab boosting'' \cite{ghosh-etal-2017-affect} for tasks such as de-biasing \cite{ma2020powertransformer}, which involves increasing the values of certain words; however, as these values are on the simplex, the softmax function necessarily decreases the values of other logits which are key to fluency such as function words.

==> removed.tex <==
\begin{comment}
\begin{table*}[!ht]
\small
\centering
\begin{tabular}{|@{ }p{4.0cm}@{ }|l@{ }|@{ }p{8.0cm}@{ }|@{ }l@{ }|@{ }l@{ }|@{ }l@{ }|}
\hline
Original Argument & System & Re-framed Argument & F & M & T   \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}} It is difficult to think of any\\ single act that would do \\more to restore America's\\ \textit{\color{red}soft power} than the election\\ of Obama to the presidency \end{tabular}} & BART$^{w/o}_{D+EN}$  & \begin{tabular}[c]{@{}l@{}}  It is difficult to think of any single act that would do more to \\restore America's \textit{\color{red}soft power} than the election of Obama to the \\presidency   \end{tabular}  & 3.7 & 2.3  & 3.0  \\ 
    \cline{2-6}
    & BART$^{w/o}_{EN}$  & \begin{tabular}[c]{@{}l@{}}  It is difficult to think of any single act that would do more to \\restore America's \textit{\color{blue}moral authority} than the election of Obama\\ to the presidency  \end{tabular}  &3.7 & 3.3 & 2.7\\
    \cline{2-6}
    & LEXREP & \begin{tabular}[c]{@{}l@{}}  It is difficult to think of any single act that would do more to \\restore America's \textit{\color{blue}moral standing} than the election of Obama\\ to the presidency \end{tabular}  & 3.7  & 3.3  & 2.7 \\
    \cline{2-6}
    & GST & \begin{tabular}[c]{@{}l@{}} \textit{\color{blue}Hated} it is difficult to think of any single act that would do\\ more to restore America's \textit{\color{blue}economy} than the election of\\ Obama to the presidency \end{tabular}  & 1.7 & 1.7 & 1.7  \\
    \cline{2-6}
    & ENTRUST & \begin{tabular}[c]{@{}l@{}}  It is difficult to think of any single act that would do more to \\restore America's \textit{\color{blue}diplomatic credibility} than the \\election of Obama to the presidency \end{tabular}  & \textbf{4.3} & \textbf{3.7}  & \textbf{4.0} \\
    \cline{2-6}
    & HUMAN & \begin{tabular}[c]{@{}l@{}}  It is difficult to think of any single act that would do more to \\restore America's \textit{\color{blue}political and economic influence} than the \\election of Obama to the presidency \end{tabular}  & 4.0 & 3.3 & 2.7 \textbf{}  \\
    \cline{2-6}
    \hline\hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}} Investors receive tax benefits\\ on capital gains that they\\ reinvest into Opportunity \\Zone through \textit{\color{red}investment}\\ \textit{\color{red}vehicles} called Qualified\\ Opportunity Funds
 \end{tabular}} & BART$^{w/o}_{D+EN}$ & \begin{tabular}[c]{@{}l@{}} Investors receive \textit{\color{blue}special} benefits on capital gains that they \\reinvest into Opportunity Zones through \textit{\color{red}investment vehicles} \\called Qualified Opportunity Funds  \end{tabular}  & \textbf{4.7}  & 3.3 & 3.0  \\
    \cline{2-6}
    & BART$^{w/o}_{EN}$ & \begin{tabular}[c]{@{}l@{}} Investors receive tax benefits on capital gains that they\\ reinvest into Opportunity Zones through \textit{\color{blue}special trust account} \\called Qualified Opportunity Funds \end{tabular}  & 4.3 & 2.7 & 3.3  \\
    \cline{2-6}
    & LEXREP & \begin{tabular}[c]{@{}l@{}}Investors receive tax benefits on capital gains that they reinvest\\ into Opportunity Zones through \textit{\color{blue}special funds} called Qualified \\Opportunity Funds \end{tabular}  & 3.3  & 3.0 & 1.7  \\
    \cline{2-6}
    & GST & \begin{tabular}[c]{@{}l@{}}  Investors receive \textit{\color{blue}income} tax benefits on capital gains that\\ they reinvest into \textit{\color{blue}white opportunity zones} through Qualified \\Opportunity Funds  \end{tabular}  & 1.7 & 2.7 & 1.7  \\
    \cline{2-6}
    & ENTRUST & \begin{tabular}[c]{@{}l@{}} Investors receive tax benefits on capital gains that they reinvest\\ into Opportunity Zones through \textit{\color{blue}special wealth} \textit{\color{blue}accounts} \\called Qualified Opportunity Funds  \end{tabular}  & 4.0 & \textbf{3.7}  & \textbf{3.7}  \\
    \cline{2-6}
    & HUMAN & \begin{tabular}[c]{@{}l@{}} Investors receive tax benefits on capital gains that they reinvest\\ into Opportunity Zones through \textit{\color{blue}financial} \textit{\color{blue} instruments} \\called Qualified Opportunity Funds \end{tabular}  &4.3 & \textbf{3.7}  & 1.3  \\
    \cline{2-6}
    \hline\hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}} Republican's vote against \\Trump's impeachment\\ reveals a \textit{\color{red}broken system} — \\and a democracy at real risk\\ of failure
 \end{tabular}} & BART$^{w/o}_{D+EN}$ & \begin{tabular}[c]{@{}l@{}} Republican's vote against Trump's impeachment reveals a\\ \textit{\color{red}broken} \textit{\color{red}system} — and a democracy at real risk of failure  \end{tabular}  & 1.3  & 1.7 &  3.0 \\ 
    \cline{2-6}
    & BART$^{w/o}_{EN}$ & \begin{tabular}[c]{@{}l@{}} Republican's vote against Trump's impeachment reveals a \\\textit{\color{blue}confirmation} \textit{\color{blue}bias} — and a democracy at real risk of failure \end{tabular}  & 2.7 & 1.3 & 3.0  \\
    \cline{2-6}
    & LEXREP & \begin{tabular}[c]{@{}l@{}}Republican's vote against Trump's impeachment reveals a \\\textit{\color{blue}dysfunctional} \textit{\color{blue}party} — and a democracy at real risk of failure \end{tabular}  & \textbf{3.7}  & 3.3 & 3.0  \\
    \cline{2-6}
    & GST & \begin{tabular}[c]{@{}l@{}} Republican's vote against Trump's impeachment reveals a\\ <unk> — and a democracy at real risk of failure  \end{tabular}  & 1.7 & 2.3 & 1.7  \\
    \cline{2-6}
    & ENTRUST & \begin{tabular}[c]{@{}l@{}} Republican's vote against Trump's impeachment reveals a \\\textit{\color{blue}fundamental} \textit{\color{blue}flaw} — and a democracy at real risk of failure  \end{tabular}  & \textbf{3.7} & \textbf{3.7}  & 3.3  \\
    \cline{2-6}
    & HUMAN & \begin{tabular}[c]{@{}l@{}} Republican's vote against Trump's impeachment reveals \\a \textit{\color{blue}flawed} \textit{\color{blue}system of accountability} — and a democracy at \\real risk of failure \end{tabular}  & \textbf{3.7} &  \textbf{3.7} & \textbf{3.7}  \\
    \cline{2-6}
    \hline
\end{tabular}
\caption{Examples of generated outputs from different systems (with human re-framed argument as references) for arguments containing partisan collocations. We show average scores (over three annotators) on a 1-5 scale with 1 denotes the worst and 5 be the best.}
\label{table:all}
\end{table*}
\end{comment}

% As we evaluate on 3 separate dimensions for 900 utterances we have a total of 2700 evaluations.


\section{Results}
% \smnote{You model is ENTRUST right? So remove "best"... }
\subsection{Automatic Evaluation}
As can be seen in Table \ref{table:simscore} our model ENTRUST maintains the denotative meaning with input better ($p<.001$ using approximate randomization tests) than other systems and only marginally behind humans when it comes to arguments with partisan collocations. For Appeal to Fear or Prejudice our system maintains better denotative meaning than all systems except LEXREP ($p<.001$). It somewhat penalizes humans for changing more content than just words which makes automated metrics not reliable always\cite{novikova-etal-2017-need}. This implicates strong need for human evaluation.
% \smnote{The above paragraph is not clear this is automatic evaluation results.}

\subsection{Human Evaluation}
% \smnote{You need to point to the Table where we see the below findings right at the begining. "Table X shows results on human evaluation". For Fluency ... }
For fluency and meaning we see how the ENTRUST model is better than all the baselines ($p<.001$ using approximate randomization tests). It is further encouraging to see that the entailment step helps us in maintaining better denotative meaning (See Table \ref{table:human} Col3: Row 4 vs Row 7). 

For Fearness ratings from MTurk results,  we see that they often rate ENTRUST model to be least fearful especially in comparison to a human expert. We hypothesize this is because human judges correlate degree of fear to the amount of fear bearing words present in an argument. Sometimes, an ungrammatical generation or a re-framing which totally change the meaning will contain less fear (rating 1 meaning no fear at all) but to avoid this we explicitly asked Turkers to rate those samples as moderate so as to not bias the overall results.
\smnote{I will work a bit on the interpretation of the results above}

\section{Analysis and Discussion}

\begin{table}[]
\small
\centering
\begin{tabular}{|l|}
\hline
\begin{tabular}[c]{@{}l@{}}An Iranian government official seemed to suggest that \\President Trump’s properties  could be potential targets\\ in retaliation for the US \textit{\color{red}targeted killing} of Iranian\\ general Qassem Soleimani.\end{tabular}                  \\ \hline
\begin{tabular}[c]{@{}l@{}}An Iranian government official seemed to .... suggest that \\President Trump’s properties  could be potential targets\\ in retaliation for the US \textit{\color{blue}involvement in the execution}\\ of Iranian general Qassem Soleimani.\end{tabular}     \\ \hline\hline
\begin{tabular}[c]{@{}l@{}}A federal appeals court ordered the U.S. Department of \\Justice to turn over key portions of a memorandum\\ justifying the government's \textit{\color{red}targeted killing} of people \\linked to terrorism, including Americans\end{tabular}        \\ \hline
\begin{tabular}[c]{@{}l@{}}A federal appeals court ordered the U.S. Department of \\Justice to turn over key portions of a memorandum\\ justifying the government's \textit{\color{blue}extrajudicial execution} of \\people linked to terrorism, including Americans\end{tabular} \\ \hline
\end{tabular}
\caption{Different Re-framed arguments by ENTRUST model based on same collocation}
\label{table:context}
\end{table}


% BART$^{w/o}_{D+EN}$ and BART$^{w/o}_{EN}$ models often fail to retain the denotation. For example changing \textit{bloody} to \textit{steady} or \textit{long} does reduce the Appeal to fear but does not keep the meaning intact. The LEXREP model on the other hand keeps the meaning intact as expected from a MLM to infill a contextual word relating to `War" however , this still fail to remove the fear completely. The ENTRUST model on the other hand uses the framing of \textit{difficult} which encompasses the struggles of a ``War", maintains the same denotative meaning, while makes it less fearful by avoiding strongly negative lexical terms like \text{painful} or \textit{bloody}.




%\newcite{Chong2007FramingT} define framing as “when (often small) changes in the presentation of an issue or an event produce (sometimes large) changes of opinion.”  Although researchers have studied the effects of framing on these opinion changes \cite{field2018framing,pryzant2020automatically}, our work is the first to use lexical framing in generation for positive framing effects.

The effects of lexical framing have been studied for social and political issues, although our work is the first to use lexical framing in generation for positive framing effects. \citet{field2018framing} proposed new ways to identify subtle media manipulation strategies at the intersection of agenda-setting and framing.  \citet{demszky2019analyzing} show how social media discussion of mass shootings is highly polarized politically and that this polarization is primarily driven by partisan differences in framing rather than topic choice.  \citet{tyagi2020computational} discussed how a major political party in India used polarized hashtags and called for escalation of conflict more so than politicians from other parties. \citet{khudabukhsh2020we} use modern machine translation methods to provide an interpretable framework to understand polarization and the differences between political framing at the granularity of words. \citet{pryzant2020automatically} rely on Wikipedia edits that removed various framings, presuppositions, and attitudes from biased sentences and train a sequence to sequence model to neutralize such biases. These works encourage computational applications of natural language processing to reframe arguments for better lexical choice.

While our focus is on lexical framing, other work has investigated the identification of other types of frames and their effects. \newcite{greene-resnik-2009-words} studied \textit{syntactic} framing, finding a link between implicit sentiment and synactic packaging (e.g. the difference between active and passive voice). Previous studies have also involved \textit{emphasis} framing -- \newcite{ding-pan-2016-personalized} find that emphasizing aspects of products given personal information is more effective for content selection in advertisements. Other research has involved \textit{issue} framing -- \newcite{ajjour-etal-2019-modeling} and \newcite{hartmann-etal-2019-issue} use an argument-specific set of frames, such as economics, feasibility, and safety,with \newcite{ajjour-etal-2019-modeling} predicting frames using multi-task learning and \newcite{hartmann-etal-2019-issue} clustering frames in a latent semantic space. \newcite{cano-basave-he-2016-study} leverage \textit{semantic} frames for distant labeling of arguments in political debates.\newcite{Musi2019FramingFS} study the use of semantic frames in fracking debates, finding that evidence and reasoning are among the most common.\newcite{DBLP:journals/pacmhci/AugustOTSR18} also use a targeted set of frames and find that alternative slogans in advertisements improve self-selection for experimental online studies.

Finally, our work is also related to style transfer and controllable generation. Much of the work in ``style transfer'' has referred to changing the sentiment of a statement, which changes the truth condition and thus the denotative meaning. Sentiment is often explicitly marked and thus approaches such as deleting and replacing lexical markers are effective \cite{li-etal-2018-delete, sudhakar-etal-2019-transforming},
although our experiments showed the difficulty of applying these techniques to our task.
To control text generation by limiting contradictions, \citet{pasunuru2017reinforced} use %address the issue of contradiction in text generation by using
an entailment score as a reward in Reinforcement Learning, ensuring that a generated text is logically implied (i.e., is a paraphrase or directed partial match with) by the ground-truth text. \citet{holtzman2018learning} utilize a discriminative model trained on SNLI \cite{bowman2015large} to complement an RNN generator and guide the decoding process to improve contradictions in generation. We experimented with both these approaches, especially the approach of \citet{holtzman2018learning} even with MNLI to account for entailment in text generation, however none of them yielded better results than our method. Other approaches have explored ``vocab boosting'' \cite{ghosh-etal-2017-affect} for tasks such as de-biasing \cite{ma2020powertransformer}, which involves increasing the values of certain words; however, as these values are on the simplex, the softmax function necessarily decreases the values of other logits which are key to fluency such as function words.
